Irreducibility of enumerable betting strategies

We study the problem of whether a betting-strategy can be decomposed into an equivalent set of simpler betting-strategies, such as betting-strategies that bet on a restricted set of stages or bet on a restricted of favorable outcomes. We show that the class of effectively enumerable betting-strategies has irreducible members which cannot be decomposed into an equivalent set of simpler betting-strategies. We answer questions of Kastermans and Hitchcock by constructing a real on which no kastergale (which is a left-c.e. supermartingale whose favorable outcomes are effectively determined) succeeds, but some unrestricted left-c.e. supermartingale succeeds on it. We generalize a result of Muchnick by showing that there is a non-1-random real such that no muchgale (which is a left-c.e. supermartingale who does not bet on certain stages) succeeds on it. Our methodology is then used to obtain further irreducibility results, strongly supporting a conjecture that if a natural class of left-c.e. supermartingales defines 1-randomness, then a single member of that class can do so. In another word, the class of left-c.e. supermartingales cannot be reduced to a simpler, natural subclass of it. For example, we show that there is a non-1-random real such that no kastergale or muchgale succeeds on it.

==> generalizebetting3combine-property.tex <==
%\def\dominationeffective{domination-effective}
\def\shrinkinginvariant{subsequence-closed}
%We say $\mcal{M}$ is \emph{effective} iff membership $ M[\leqslant t] \in\mcal{M}$ is decidable.
 We say $\mcal{M}$ is \emph{non decreasing} if for each $ M[\leqslant t] \in\mcal{M}$,
$M[\h t]$ dominates $M[\h t-1]$ for all $1\leq \h t\leq t$.
We say $\mcal{M}$ is \emph{\homogeneous} iff:
for every $\rho\in 2^{<\omega}$, let $h_\rho$ denote the isomorphism
$\sigma\mapsto \rho\sigma$, we have
$ M[\leqslant t]\in\mcal{M}$ implies $ M[\leqslant t]\circ h_\rho\in\mcal{M}$.
We say $\mcal{M}$ is \emph{\shrinkinginvariant} iff
for every $M[\leqslant   t]\in\mcal{M}$,
every $ t_0<\cdots<t_{s-1}\leq t$,
$(M[t_0],\cdots,M[t_{s-1}])\in\mcal{M}$
%and for every $t'<t$,
%  $(M[0],\cdots, M[t'-1], M[t'],\cdots,M[t'],M[t'+1],\cdots,M[t])\in\mcal{M}$
\footnote{\label{singfootnote0} The \shrinkinginvariant\ together with
$\Pi_1^0$-class of $\mcal{M}$ ensures that the winning strategy of \alice\ is computable,
which is needed when applying the winning strategy in,
say, the proof of Theorem \ref{singth3}.
To this end,
it suffices that \alice\  computably knows all the possible action of \baby\ at round $t$
given the game history.
Note that $\Pi_1^0$-class of $\mcal{M}$
is not enough.
Because when \alice\ plays against computable $\mcal{M}$-gales
and  enumerates a string  (at time $t$),
the valid action of \baby\ may come very late, say at time $\h t$
where $\h t$ is much larger than $t$.
For example, consider the class $\{M^*\}$ where $M^*$ is the universal
left-c.e. supermartingale. For this class,
\alice\ has a winning strategy for the $(c,n,1)$-$\mcal{M}$-game
played at $[\rho]^\preceq\cap 2^{\leq n+|\rho|}$
by enumerating one string in $[\rho]^\preceq\cap 2^{n+|\rho|}$, provided $M^*(\rho)<c$. But the winning  strategy is not computable
(uniformly in $\rho$) as
the class is not \shrinkinginvariant.
%Also note that \shrinkinginvariant\ together with effectiveness
%promises that we can computably list all members of computable $\mcal{M}$-gales.
}. 
We say $\mcal{M}$ is \emph{scale-closed} iff for every $M[\leqslant t]\in\mcal{M}$,
every $c>0$, $cM[\leqslant t]\in\mcal{M}$.
Abusing terminology, we say $\mcal{M}$ is \emph{$\Pi_1^0$-class} iff for every $t\in\omega$,
the set of $M[\leqslant t]\in\mcal{M}$ is a $\Pi_1^0$-class uniformly in $t$.

==> generalizebetting4combine.tex <==



\section{Subclasses of left-c.e. supermartingale}
\label{singsecgen}

We address the question: is there a proper subclass
of left-c.e. supermartingale defining 1-randomness.
First, we need to formalize the question.
%A set $\mcal{M}$ of \emph{\supermartingaleapp} is a set of finite sequences
% $(M[0],\cdots,M[t])$ (denoted as $M[\leqslant t]$)
%of supermartingales.
%Let $\lce$ denote the set of $M[\leqslant t]$ so that $M[\leqslant t]$ is non decreasing
%with respect to $t$.
%We say $\mcal{M}$ is \emph{left-c.e.} if $\mcal{M}\subseteq \lce$.
A   \emph{ \supermartingaleapp s}
 is a sequence $M[\leqslant t] = (M[0],\cdots,M[t])$
 of supermartingales.
In this section, we use  $\mcal{M}$
to denote a class of \supermartingaleapp s.
An \emph{$\mcal{M}$-gale} is an infinite sequence $(M[t]:t\in\omega)$
such that $M[\leqslant t]\in \mcal{M}$ for each $t\in\omega$
and   $\lim_{t\rightarrow\infty} M[t](\sigma)$ exist for all $\sigma\in 2^{<\omega}$;
it is \emph{computable} iff $(M[t]:t\in\omega)$ is computable.

 \begin{example}
 For muchgale, let $\mcal{M}_l$ be the class of non decreasing
 \supermartingaleapp s\
 $M[\leqslant t]$ such that
 for some $i<l$, $M[\h t]$ is $(l,i)$-\betting\ for all $\h t\leq t$.
 Let $\mcal{M} = \cup_l \mcal{M}_l$, then muchgale is computable $\mcal{M}$-gale.
 For kastergale,
 let $\mcal{M}$ be the class of non decreasing \supermartingaleapp\
 $M[\leqslant t]$ such that
 for every $\sigma\in 2^{<\omega}$,
 if there is a $\h t\leq t$ such that $M[\h t](\sigma0)>M[\h t](\sigma 1)$,
 then for every $\h t\leq t$, $M[\h t](\sigma0)\geq M[\h t](\sigma 1)$.
 Then kastergale is computable $\mcal{M}$-gale.


\end{example}

Given a class $\mcal{M}$ of   \supermartingaleapp s,
we can always define the     analog
of game \ref{singdef2}.
\begin{definition}[$(c,n,  k)$-$\mcal{M}$-game]
\label{singdefgen0}
At each round $t\in\omega$, \alice\ firstly presents a   set $A[t]\subseteq  2^{  n}$
with $A[t]\supseteq A[t-1]$;
then \baby\ presents $(M_j[t],j<k)$ with  $ M_j[\leqslant t] \in\mcal{M}$ for each $j<k$ such that:
\begin{itemize}

\item for every $\sigma\in A[t]$,
 $|| \Mb[t](\h\sigma)||_1\geq 1 $ for some $\h\sigma\preceq\sigma$;
%\item $ M_j[\leqslant t] \in\mcal{M}$.
%(we set $M_j[-1]\equiv 0$)


\end{itemize}
\alice\ wins the game if for some $t$, $||\Mb[t](\emptyset)||_1\geq  c$.


\end{definition}
\input{generalizebetting3combine-property.tex}
%We will consider subclass of left-c.e. supermartingales that is  somewhat homogeneous.
%We say $\mcal{M}$ is \emph{scale-closed} iff for every $(M[\leqslant t],q[\leqslant t])\in\mcal{M}$,
%every $c>0$, $(cM[\leqslant t],q[\leqslant t])\in\mcal{M}$\footnote{Since $q[t]$ is a
%set of sequences $(\h M[t]: t\in\omega)$, so $cq[t]$ is the set of sequences
%$(c\h M[t]:t\in\omega)$.}.
We say $\mcal{M}$ is \emph{\homogeneous} iff:
for every $\rho\in 2^{<\omega}$, let $h_\rho$ denote the isomorphism
$\sigma\mapsto \rho\sigma$, we have
$ M[\leqslant t]\in\mcal{M}$ implies $ M[\leqslant t]\circ h_\rho\in\mcal{M}$.
Abusing terminologies, we say $\mcal{M}$ is \emph{$\Pi_1^0$-class}
if for every $t\in\omega$, the set of $M[\leqslant t]\in\mcal{M}$
is a $\Pi_1^0$-class uniformly in $t$.
%\footnote{Here $q[t]\circ h_\rho$ is the set of sequences $(\h M[t]\circ h_\rho:t\in\omega)$.}.
\begin{remark}\label{singremhomo}
The \stronghomogeneity\ property is implicitly used in all  ingredients
(as all those finite games are defined on $[\emptyset]^\preceq\cap 2^{\leq n}$ instead of
$[\rho]^\preceq\cap 2^{\leq |\rho|+n}$).
%With that said, the above defined \homogeneity\ is still stronger than what we need.
%But we will not discuss that since all naturally defined \supermartingaleapp s classes are \homogeneous.
%The  effectiveness are used in  the proof of Theorem   \ref{singth3}   using Lemma \ref{singlem41};
%other than ensuring the winning strategy of \alice\ is computable (see footnote \ref{singfootnote0}),
%it   also promises that we can computably list all members of computable $\mcal{M}$-gales.
\end{remark}


Let classes of \supermartingaleapp\ $(\mcal{M}_l:l\in\omega)$ be $\Pi_1^0$-class (uniformly in $l$),
\shrinkinginvariant,  non decreasing and homogeneous with $\mcal{M}_l\subseteq \mcal{M}_{l+1}$ for all $l\in\omega$;
and $\mcal{M} = \cup_l \mcal{M}_l$.
As  the proof of Theorem \ref{singth3} using Lemma \ref{singlem43},
\begin{claim}\label{singgenclaim1}
Suppose for every  $l\in\omega$,
every $ c<1, \varepsilon>0$ and $k\in\omega$,
 there is an $n\in\omega$, such that
 \alice\ has a winning strategy
for   $(c,n,  k)$-$\mcal{M}_l$-game \ref{singdefgen0} such that
$\m(A)\leq \varepsilon$.
Then there is a non-1-random real $x\in 2^\omega$
on which no computable $\mcal{M}$-gale succeeds.
\end{claim}
As commented in remarks \ref{singrem1},\ref{singrem2},\ref{singrem3} and \ref{singremhomo}
(that iteration, dynamic goal, restriction and reducing to \variancee\ game only concern
non decreasing, supermartingale  and \homogeneity\ of $\mcal{M}$),
the winning strategy of $\mcal{M}$-game \ref{singdefgen0} (with arbitrary small cost)
is reduced to the winning strategy of the corresponding \variancee\
game (with a cost smaller than $1$).
\begin{definition}[\variancee\ $(a,\Delta ,m,k)$-$\mcal{M}$-game]
\label{singdefgen2}
At each round $t\in\omega$, \alice\ firstly presents a prefix-free set $A[t]\subseteq  2^{ m}$
with $A[t]\supseteq A[t-1]$;
then \baby\ presents $(M_j[t],j<k)$ with $ M_j[\leqslant t] \in\mcal{M}$ for each $j<k$ such that:
\begin{itemize}

\item for every $\sigma\in A[t]$,
 $||\Mb[t]( \sigma)||_1\geq 1 $;
%\item $ M_j[\leqslant t] \in\mcal{M}$.
%\item $||\Mb[t]( \rho)||_1\leq 1+\delta$ for all $ \rho\in  2^{\leq m}$.
%(we set $M_j[-1]\equiv 0$)


\end{itemize}
\alice\ wins the game if for some $t$,
\begin{itemize}
\item (type-(a)) either $1-|| \Mb[t](\emptyset)||_1\leq  \frac{1}{a} (1-\m(A[t]))$;

\item (type-(b))  or $\variance(\Mb[t]|A[t])\geq \Delta$
\end{itemize}

\end{definition}


As commented in remark \ref{singrem-1},
a winning strategy for \variancee\ game \ref{singdefgen2} is
reduced to the special case $k=1$ and
that reduction only depends on non decreasing, supermartingale
and \homogeneity.
i.e., Let $\mcal{M}$ be non decreasing and \homogeneous.
\begin{claim}\label{singgenclaim0}
Suppose for every  $a>0$,
there are $m\in\omega$, $\Delta>0$
such that
\alice\ has a winning strategy
for
  \variancee\ $(a,\Delta ,m,1)$-$\mcal{M}$-game \ref{singdefgen2}
such that $\m(A)<1$.
Then for
every $ c<1, \varepsilon>0$ and $k\in\omega$,
there is an $n\in\omega$ such that
 \alice\ has a winning strategy
for   $(c,n,  k)$-$\mcal{M}$-game \ref{singdefgen0} such that
$\m(A)\leq \varepsilon$.
\end{claim}

We already demonstrated how to defeat a single
kastergale (in the \variancee\ game) in section \ref{singsec100}.
Thus, to prove Theorem \ref{singth5},
it suffices to show how to defeat a single muchgale.
However, this is obvious. Because for the class of $(l,i)$-betting
supermartingales,
\alice\ could simply enumerate the set $\{\sigma\in 2^n:\sigma(i) = 0\}$
(which forces $M[t](\emptyset)\geq 1$).
By Claim \ref{singgenclaim1} and \ref{singgenclaim0}, we immediately have
\singthunion*




There is one more step to verify conjecture (\ref{singconj0}).
In the actual game, the Martin-L\"{o}f player does not enumerate
strings at a fixed level $n$. Therefore, we consider
\begin{definition}[weakly-restricted dynamic $(a, m,k)$-$\mcal{M}$-game]
\label{singdefgen3}
Rules:
the same as \variancee\ $(a,\Delta ,m,k)$-$\mcal{M}$-game \ref{singdefgen2}
except that $A[t]\subseteq 2^{\leq m}$ is a finite \pf\ set (instead of $A[t]\subseteq 2^m$).
Winning criterion of \alice:  type-(a) winning criterion of \variancee\ $(a,\Delta ,m,k)$-$\mcal{M}$-game \ref{singdefgen2}.

\end{definition}

Note that   definition \ref{singdefgen3} makes sense when $m=\omega$. We say $\mcal{M}$
is \emph{closed} if for every $M_0[\leqslant t],M_1[\leqslant t],\cdots\in\mcal{M}$,
  the pointwise limit of $M_0[\leqslant t],M_1[\leqslant t],\cdots$
   \footnote{The pointwise limit of $M_0[\leqslant t],M_1[\leqslant t],\cdots$
   refers to $M[\leqslant t]$ such that for every $\h t\leq t,\sigma\in 2^{<\omega}$,
   we have $\lim_{k\rightarrow\infty}M_k[\h t](\sigma) = M[\h t](\sigma)$.
  Of course, if $\mcal{M}$ is a $\Pi_1^0$-class, then it is closed.} (if it exists) is also in $\mcal{M}$.

Let $a>0$,$k\in\omega$, $\varepsilon<1$; let $\mcal{M}$ be   closed.
\begin{claim}
\label{singgenclaim3}
Suppose \alice\ has a winning strategy for   $(a ,\omega,k)$-$\mcal{M}$-game \ref{singdefgen3}
such that $\m(A)\leq \varepsilon$.
Then,
there is an $m\in\omega$ such that
 \alice\ has a winning strategy for   $(a/2, m,k)$-$\mcal{M}$-game \ref{singdefgen3}
such that $\m(A)\leq \varepsilon$.
\end{claim}
\begin{proof}
\def\ws{\mcal{W}}

Although the details are tedious, the proof simply follows by
 compactness.
 Suppose otherwise. Then, for every $m\in\omega $, there is a ``winning strategy"
 of \baby\
 for   $(a/2, m,k)$-$\mcal{M}$-game \ref{singdefgen3}
  \footnote{The strategy prevents \alice\ from winning
  $(a/2, m,k)$-$\mcal{M}$-game \ref{singdefgen3} with $\m(A)\leq \varepsilon$.}.
 Note that winning strategy of \baby\ is nothing but a function $\ws_m$
 mapping a game history $A[t],\Mb[\leq t-1]$ to an action $\Mb[t]$.
 We may assume that $\ws_m$ is continuous with respect to $\Mb[\leq t-1]$.
 Then, take $\ws$ to be the (pointwise) limit
 of a subsequence of $(\ws_m:m\in\omega)$.
 By closeness of $\mcal{M}$, $\ws$  also maps a game history $A[t],\Mb[\leq t-1]$
 to a valid action $\Mb[t]$ of \baby.
 To derive a contradiction, it suffices to show
  that $\ws$  prevents \alice\ from winning the
  $(a,\omega,k)$-$\mcal{M}$-game \ref{singdefgen3}
such that $\m(A)\leq \varepsilon$.

Suppose on the contrary \alice\ wins the   $(a,\omega,k)$-$\mcal{M}$-game \ref{singdefgen3}
by round $t$ such that $\m(A[t])\leq \varepsilon$;
suppose $A[t]\subseteq 2^{\leq m}$.
 Let $m^*\geq m$ be sufficiently large
so that $\ws_{m^*}$ is very close to $\ws$ (depending on $a,\varepsilon$). Since $\ws_{m^*}$ is a winning strategy of
\baby\ (for  $(a/2, m,k)$-$\mcal{M}$-game \ref{singdefgen3})
and since $\ws$ is very close to $\ws_{m^*}$ and $\ws_{m^*}$ is continuous,
 we have $\Mb[t]$ is very close to the action of \baby\ (at round $t$) given by $\ws_{m^*},A[\leq t]$.
 Thus,
 \begin{align}\nonumber
 &1-|| \Mb[t](\emptyset)||_1\geq  \frac{2}{a} (1-\m(A[t]))-o(1)
>\frac{1}{a} (1-\m(A[t])).
 \end{align}
Thus, contradicting to \alice\ wins  the   $(a,\omega,k)$-$\mcal{M}$-game \ref{singdefgen3}
by round $t$.
\end{proof}

\def\scaleclosed{scale-closed}
Now we formalize conjecture (\ref{singconj0}) and prove it.
We say   $\mcal{M}$ is \emph{\scaleclosed}
if for every  $M[\leqslant t]\in\mcal{M}$, every $c>0$,
$cM[\leqslant t]\in\mcal{M}$;
we say $\mcal{M}$ is \emph{Markovian}
if for every $M[\leqslant t],\h M[\leqslant t]\in\mcal{M}$, every $\rho\in 2^{<\omega}$,
suppose $\h M[\h t](\emptyset)\leq M[\h t](\rho)$ for all $\h t\leq t$,
then
replacing $M[\leqslant t]\uhr [\rho]^\prec$ by $\h M[\leqslant t]$ still gets a member of $\mcal{M}$. i.e.,
 Let $\t M[\leqslant t]$ be such that $\t M[\leqslant t]\uhr (2^{<\omega}\setminus [\rho]^\prec)
 \equiv M[\leqslant t]\uhr (2^{<\omega}\setminus [\rho]^\prec)$ and $\t M[\leqslant t]\uhr [\rho]^\prec
  \equiv \h M[\leqslant t]\circ h_\rho^{-1}$, we have $\t M[\leqslant t]\in\mcal{M}$.
\begin{theorem}
\label{singgenth0}
Let classes of \supermartingaleapp\ $(\mcal{M}_l:l\in\omega)$ be $\Pi_1^0$-class (uniformly in $l$),
\shrinkinginvariant,  non decreasing, homogeneous,
Markovian   and \scaleclosed\
such that $\mcal{M}_l\subseteq \mcal{M}_{l+1}$ for all $l\in\omega$
and $(M_0,M_0,\cdots)\in\mcal{M}_0$ (where $M_0\equiv 0$);
let $\mcal{M} = \cup_l\mcal{M}_l$.
We have: computable $\mcal{M}$-gales define 1-randomness if and only if
there is one computable $\mcal{M}$-gale succeeding on all non-1-random reals.

\end{theorem}
\begin{proof}
Suppose computable $\mcal{M}$-gales define 1-randomness.
By Claim \ref{singgenclaim1}, \ref{singgenclaim0},
there is an $a>0$ such that for every $m\in\omega,\Delta>0$,
 \alice\ does not have a winning strategy for \variancee\ $(a,\Delta ,m,1)$-$\mcal{M}$-game
such that $\m(A)\leq 1/2$.
In particular, for every $m\in\omega$, \alice\ does not have a winning strategy for
$(a,m,1)$-$\mcal{M}$ game \ref{singdefgen3} such that $\m(A)\leq 1/2$
(as the rules of game \ref{singdefgen3} are the same as \variancee\ game while the winning criterion is
stronger).
By Claim \ref{singgenclaim3}, \alice\ does not have a winning strategy for
 $(2a  ,\omega,1)$-$\mcal{M}$-game \ref{singdefgen3} such that
$\m(A)\leq 1/2$. We refer to the strategy of \baby\ achieving this
as winning strategy of \baby.

Let $(V_k:k\in\omega)$ be such a universal Martin-L\"{o}f test that
for every $k\in\omega$,
$V_k$ is prefix-free and
every $\rho\in V_k$, $\m(V_{k+1}|\rho)\leq 1/2$.
Note that by taking $(V_0[t]:t\in\omega)$ (the approximation of c.e. set $V_0$)
as the action of \alice, using the winning strategy of \baby,
we can compute a $(M[t]:t\in\omega)\in\mcal{M}$
such that
let $M = \lim_{t\rightarrow\infty }M[t]$, we have
$M(\rho)\geq 1$ for all $\rho\in V_0$ and $M(\emptyset)\leq 1-\frac{1}{2a}(1-\m(V_0))
\leq c$ where $c= 1-\frac{1}{4a}$.
Now for each $\rho\in V_0$, apply the winning strategy of \baby\
on the game over $\rho$ (where the action of \alice\ is given
by $(V_1[t]\cap [\rho]^\preceq:t\in\omega)$), by scaling, we can additionally achieve that
$M(\rho)\geq 1/c$ for all $\rho\in V_1$
\footnote{
We need the \scaleclosed\ of $\mcal{M}$
 to show that  \baby\ has a winning strategy
for the scaled  $(a, \omega,1)$-$\mcal{M}$-game \ref{singdefgen3}.
Before playing over  $\rho\in V_0$
against the actions of $V_1$,  we set $M[t](\rho)=0$ for all $\rho\in [V_0[t]]^\prec$
(which is feasible by Markovian of $\mcal{M}$
and since $(M_0,M_0,\cdots)\in\mcal{M}$).
We   need to glue
the actions of \baby\ (against different $V_k$) together to form $(M[t]:t\in\omega)$.
This is where we use the Markovian of $\mcal{M}$.}
without sabotaging $M(\emptyset)\leq c$.
In the end, for every $k\in\omega$ and $\rho\in V_k$, $M(\rho)\geq 1/ c^{k-1}$.
Thus we are done.

\end{proof}


